DAM-GT: Dual Positional Encoding-Based Attention Masking Graph Transformer for Node Classification

Neighborhood-aware tokenized graph Transformers have recently shown great potential for node classification tasks. Despite their effectiveness, our in-depth analysis of neighborhood tokens reveals two critical limitations in the existing paradigm. First, current neighborhood token generation methods fail to adequately capture attribute correlations within a neighborhood. Second, the conventional self-attention mechanism suffers from attention diversion when processing neighborhood tokens, where high-hop neighborhoods receive disproportionate focus, severely disrupting information interactions between the target node and its neighborhood tokens. To address these challenges, we propose DAM-GT, Dual positional encoding-based Attention Masking graph Transformer. DAM-GT introduces a novel dual positional encoding scheme that incorporates attribute-aware encoding via an attribute clustering strategy, effectively preserving node correlations in both topological and attribute spaces. In addition, DAM-GT formulates a new attention mechanism with a simple yet effective masking strategy to guide interactions between target nodes and their neighborhood tokens, overcoming the issue of attention diversion. Extensive experiments on various graphs with different homophily levels as well as different scales demonstrate that DAM-GT consistently outperforms state-of-the-art methods in node classification tasks.

==> body/02rw.tex <==

\subsection{Graph Neural Network}
GNNs have been effective approaches for node classification, while neighborhood aggregation is the most important module in GNN-based methods.
Prior GNNs~\cite{gcn,gat,graphsage} focus on aggregating information of immediate neighbors.
In addition to immediate neighbors, follow-up methods aim to capture structural information beyond the local neighborhood. 
A line of approaches~\cite{mixhop,jknet,gcnii} introduces the residual connection into GNNs.
Another line of methods~\cite{pt,pamt,ncgnn,appnp,sgc,gprgnn} adopts the decoupled design to achieve efficient information aggregation of multi-hop neighborhoods~\cite{rlp}. 

Besides aggregating neighborhood information based on the topology space, several studies~\cite{simpGNN,amgcn,geomgcn} explore the aggregation operation in the semantic feature space.
The key idea of the aggregation operation in these methods is to aggregate information of nodes with high similarity according to the input feature.

Previous GNN-based studies have shown that both topology and semantic features are important to learn informative node representations from the input graph.
This phenomenon motivates us to design a new positional encoding that not only captures the structural information, but also preserves the semantic information in the attribute feature space for effective node representation learning.


\subsection{Graph Transformer}
We divide existing graph Transformers for node classification into two groups according to the model input~\cite{ntformer}, \ie, graph-based approaches and token-based approaches.

Graph-based approaches require the whole graph as input for Transformers. Approaches of this category develop various strategies, such as positional encoding~\cite{gt,gps} and GNN-style modules~\cite{gps,nodeformer,sgformer,gapformer,cob}, to encode the graph structure information since Transformer regards the input graph as fully-connected, naturally ignoring the graph structural information. 

Though effective, a recent study~\cite{cob} has theoretically proved that directly applying the self-attention on graphs would cause the over-globalization issue, inevitably limiting the model performance.
Unlike previous methods, token-based approaches~\cite{gophormer,ansgt,nagformer,vcr} first transform the input graph into short independent token sequences. Then, the generated token sequences are fed into the Transformer to learn node representations.
This strategy naturally overcomes the over-globalization issue. Besides, the training cost is greatly reduced by applying the mini-batch training strategy, effectively improving scalability to handle graphs of arbitrary scales, which is important for node classification task.

Some methods select nodes with high similarity as tokens according to different sampling strategies, such as Top-$k$ sampling~\cite{ansgt} and random walk-based sampling~\cite{gophormer,ansgt}.
In addition to node-aware tokens, previous methods~\cite{nagformer,vcr} utilize the propagation strategies, such as random walk~\cite{nagformer} and personalized PageRank~\cite{vcr} to transform the multi-hop neighborhoods into token sequences.
Since neighborhood-aware tokens can comprehensively preserve the local topology information~\cite{vcr}, neighborhood token-based methods~\cite{nagformer,vcr} show promising performance in node classification.

Nevertheless, we observe that large-hop neighborhood tokens can interfere with the distribution of attention scores due to the characteristics of neighborhood tokens.
This issue weakens the interactions between the target nodes and multi-hop neighborhoods, hindering learning node representations from neighborhood tokens effectively.
Hence, we propose a new attention mechanism that adopts the masking strategy to ensure efficient information aggregation between the target node and its neighborhood tokens.

